Chordal Sparsity for SDP-based Neural Network Verification

Neural networks are central to many emerging technologies, but verifying their correctness remains a major challenge. It is known that network outputs can be sensitive and fragile to even small input perturbations, thereby increasing the risk of unpredictable and undesirable behavior. Fast and accurate verification of neural networks is therefore critical to their widespread adoption, and in recent years, various methods have been developed as a response to this problem. In this paper, we focus on improving semidefinite programming (SDP) based techniques for neural network verification. Such techniques offer the power of expressing complex geometric constraints while retaining a convex problem formulation, but scalability remains a major issue in practice. Our starting point is the DeepSDP framework proposed by Fazlyab et al., which uses quadratic constraints to abstract the verification problem into a large-scale SDP. However, solving this SDP quickly becomes intractable when the network grows. Our key observation is that by leveraging chordal sparsity, we can decompose the primary computational bottleneck of DeepSDP -- a large linear matrix inequality (LMI) -- into an equivalent collection of smaller LMIs. We call our chordally sparse optimization program Chordal-DeepSDP and prove that its construction is identically expressive as that of DeepSDP. Moreover, we show that additional analysis of Chordal-DeepSDP allows us to further rewrite its collection of LMIs in a second level of decomposition that we call Chordal-DeepSDP-2 -- which results in another significant computational gain. Finally, we provide numerical experiments on real networks of learned cart-pole dynamics, showcasing the computational advantage of Chordal-DeepSDP and Chordal-DeepSDP-2 over DeepSDP.

==> authors.tex <==


% \setlength{\columnsep}{2pt}%

\begin{wrapfigure}{l}{0.2\textwidth}
  \begin{center}
    \includegraphics[width=1.0\linewidth]{author_pictures/anton.jpg}
  \end{center}
\end{wrapfigure}

% \includegraphics[width=100px]{author_pictures/anton.jpg}
Anton Xue is currently a Ph.D. student in the Computer and Information Science Department at the University of Pennsylvania. He received a B.S. degree in Mathematics and a B.S. degree in Computer Science from Yale University in 2019. He received the National Science Foundation Graduate Research Fellowship in 2019. His research interests lie at the intersection of machine learning, optimization, formal methods, and explainability.


\begin{wrapfigure}{l}{0.2\textwidth}
  \begin{center}
    \includegraphics[width=1.0\linewidth]{author_pictures/lars.jpg}
  \end{center}
\end{wrapfigure}
Lars Lindemann is currently an Assistant Professor in the Thomas Lord Department of Computer Science at the University of Southern California, where he is a member of the Robotics and Autonomous Systems Center and the Center for Autonomy and Artificial Intelligence. Between 2020 and 2022, he was a Postdoctoral Fellow in the Department of Electrical and Systems Engineering at the University of Pennsylvania. He received a Ph.D. degree in Electrical Engineering from KTH Royal Institute of Technology in 2020.  His research interests include systems and control theory, formal methods, and autonomous systems. Professor Lindemann received the Outstanding Student Paper Award at the 58th IEEE Conference on Decision and Control and the Student Best Paper Award (as a co-advisor) at the 60th IEEE Conference on Decision and Control. He was a finalist for the Best Paper Award at the 2022 Conference on Hybrid Systems: Computation and Control and for the Best Student Paper Award at the 2018 American Control Conference.


\begin{wrapfigure}{l}{0.2\textwidth}
  \begin{center}
    \includegraphics[width=1.0\linewidth]{author_pictures/rajeev.jpg}
  \end{center}
\end{wrapfigure}
Rajeev Alur is the Zisman Family Professor of Computer and Information Science and the Founding Director of ASSET (Center for AI-Enabled Systems: Safe, Explainable, and Trustworthy) at the University of Pennsylvania. He obtained his bachelor's degree in computer science from IIT Kanpur in 1987 and PhD in computer science from Stanford University in 1991. Before joining Penn in 1997, he was with the Computing Science Research Center at Bell Labs. His research is focused on formal methods for system design and spans artificial intelligence, cyber-physical systems, distributed systems, logic in computer science, machine learning, and programming languages. He is a Fellow of the AAAS, a Fellow of the ACM, a Fellow of the IEEE, an Alfred P. Sloan Faculty Fellow, and a Simons Investigator. He was awarded the inaugural CAV (Computer-Aided Verification) award in 2008, ACM/IEEE Logic in Computer Science (LICS) Test-of-Time award in 2010, the inaugural Alonzo Church award by ACM SIGLOG / EATCS / EACSL / Kurt Goedel Society in 2016, Distinguished Alumnus Award by IIT Kanpur in 2017 for his work on timed automata. Prof. Alur has served as the chair of ACM SIGBED (Special Interest Group on Embedded Systems), the general chair of LICS, and the lead PI of the NSF Expeditions in Computing Center ExCAPE (Expeditions in Computer Augmented Program Engineering). He is the author of the textbook Principles of Cyber-Physical Systems (MIT Press, 2015).




==> contents/acknowledgements.tex <==
% \section*{Acknowledgements}

\paragraph*{Acknowledgements}
This work was partially funded by ONR Science of AI award N00014-20-1-2115 and a gift from AWS AI to Penn Engineering ASSET Center.

==> contents/admm.tex <==
\section{Chordally Sparse DeepSDP with ADMM}
\label{sec:admm}
So far we have developed a method to decompose DeepSDP's large semidefinite program~\eqref{eq:deepsdp-Z} into an equivalent collection of smaller ones~\eqref{eq:p2}.
This is typically desirable for solver calls, but still this is not entirely scalable because a single instance of problem~\eqref{eq:p2} must still encode the entire network.
As such, we look to large-scale convex optimization techniques like the \emph{Alternating Direction Method of Multipliers} (ADMM)~\cite{boyd2011distributed} to overcome the solver bottleneck.
In this work, we derive an algorithm based on the recent ADMM-based algorithm for chordally sparse semidefinite programs~\cite{zheng2019chordal}.
This angle has several merits.
First, ADMM-based algorithms are amenable to parallelization and distributed computation.
In addition, as an iterative method it can easily implement trade-offs between solution quality and runtime.
Furthermore,  our implementation uses relatively simple operations while achieving a performance gain.

In this section we first present some notation and properties for vectorized matrix expressions.
We then give a reformulation of problem~\eqref{eq:p2}, derive its \emph{augmented Lagrangian}, and assign the problem variables an update order.
By staggering the order of variable updates, we can more easily exploit algebraic properties for performance: it becomes possible to derive closed-form expressions for expensive computations and apply aggressive caching strategies.
We round out the section with some discussion on the theoretical and practical aspects of our algorithm.

\subsection{Vectorized Forms}
Let \(\mrm{vec} : \mbb{R}^{n \times n} \to \mbb{R}^{n^2}\) take a square matrix to vectorized stack of its columns, and similarly define its inverse \(\mrm{mat} : \mbb{R}^{n^2} \to \mbb{R}^{n \times n}\) to map a stack of columns back into a square matrix.
By convention, we will use capital letters for matrices and lower-case letters for their corresponding vectorized forms.
For instance, we write \(x = \mrm{vec}(X)\) and \(X = \mrm{mat}(x)\).

For each clique \(\mcal{C}_k\) as given in~\eqref{eq:Ck}, define the matrix \(H_k \coloneqq E_{\mcal{C}_k} \otimes E_{\mcal{C}_k}\) via the Kronecker product in order to satisfy the following properties,
\begin{align*}
    x_k = \mrm{vec}(E_{\mcal{C}_k} X E_{\mcal{C}_k} ^\top) = H_k x,
    \qquad
    H_k ^\top x_k = \mrm{vec} (E_{\mcal{C}_k}^\top X_k E_{\mcal{C}_k}).
\end{align*}
Also define vectorized sets of semidefinite matrices and the indicator function as
\begin{align*}
    \mcal{S}_k =
    \braces{v \in \mbb{R}^{\lvert \mcal{C}_k \rvert} : \mrm{mat}(v) \in \mbb{S}_{-} ^{\lvert \mcal{C}_k \rvert}},
    \qquad
    \delta_{\mcal{A}} (x) =
        \begin{dcases}
            0, &\enskip x \in \mcal{A} \\
            +\infty, &\enskip \text{otherwise}
        \end{dcases}
\end{align*}
Vectorizations of affine matrix-valued functions also have a convenient form.
Define \(\gamma \coloneqq \begin{bmatrix} \gamma_{\mrm{in}}^\top & \gamma_{\mrm{ac}}^\top \end{bmatrix}^\top\), and observe that
\begin{align*}
    z_{\beta} (\gamma)
    = \mrm{vec} (Z_\beta (\gamma))
    = \mrm{vec}(Z_{\beta, 0}) + \sum_{i = 1}^{N} \mrm{vec}(Z_{\beta, i}) \gamma_i
    = z_{\beta, 0} + J \gamma
\end{align*}
where \(Z_{\beta, i}\) for \(i \geq 1\) are the components of \(Z_\beta\), and whose vectorized forms \(z_{\beta, i}\) are the columns of \(J\).


\subsection{Augmented Lagrangian}
We now introduce some slack variables \(v_1, \ldots, v_p\) and reformulate~\eqref{eq:p2} as follows,
\begin{align}
\label{eq:p3}
\begin{split}
    \underset{\gamma, v_1, \ldots, v_k, z_1, \ldots, z_k}{\text{minimize}}
        &\quad \frac{1}{2} \norm{\gamma}^2
            + \delta_{\mbb{R}_+} (\gamma)
            + \delta_0 \parens{z_{\beta} (\gamma) - \sum_{k = 1}^{p} H_k ^\top v_k}
            + \sum_{k = 1}^{p} \delta_{\mcal{S}_k} (z_k) \\
    \text{subject to}
        &\quad v_k = z_k, \quad k = 1, \ldots, p
\end{split}
\end{align}
Note that this is now a minimization problem rather than a satisfiaiblity problem.
In particular, we have moved the equality and nonnegative constraints into the objective as indicator variables.
Furthermore, we introduce a \(\norm{\gamma}^2 / 2\) term to help simplify algebraic derivations later; this additional term has no impact on satisfiability because it does not alter the search space.

We proceed with formulating the augmented Lagrangian.
For the \(p\) equality constraints of~\eqref{eq:p3} we introduce the dual variables \(\lambda_1, \ldots, \lambda_p\), and for notational convenience define
\begin{align*}
    v = (v_1, \ldots, v_p),
    \quad z = (z_1, \ldots, z_p),
    \quad \lambda = (\lambda_1, \ldots, \lambda_p).
\end{align*}
The augmented Lagrangian for~\eqref{eq:p3} is parameterized by a \(\rho > 0\), and is given as
\begin{align}
\label{eq:p3-lagrangian}
\begin{split}
    L_\rho (\gamma, v, z, \lambda)
    &\coloneqq \frac{1}{2} \norm{\gamma}^2 + \delta_{\mbb{R}_+} (\gamma) + \delta_0 \parens{z_{\beta} (\gamma) - \sum_{k = 1}^{p} H_k ^\top v_k} \\
    &\quad + \sum_{k = 1}^{p} \delta_{\mcal{S}_k} (z_k)
        + \sum_{k = 1}^{p} \frac{\rho}{2} \xnorm{z_k - v_k + \rho^{-1} \lambda_k}^2
\end{split}.
\end{align}
This variant is known as the \emph{scaled} augmented Lagrangian, and other equivalent formulations exist~\cite{boyd2011distributed}.
In our algorithm we begin with zero-valued problem variables \(\gamma^{(0)}, v^{(0)}, z^{(0)}, \lambda^{(0)}\), and perform the following update steps at each iteration until a stopping condition is hit:
\begin{align}
\label{eq:admm-updates}
\begin{split}
    \gamma^{(t+1)}, v^{(t+1)}
        &= \underset{\gamma, v}{\text{update}} \enskip L_{\rho} (\gamma, v, z^{(t)}, \lambda^{(t)}) \\
    z^{(t+1)}
        &= \underset{z}{\text{update}} \enskip L_{\rho} (\gamma^{(t+1)}, v^{(t+1)}, z, \lambda^{(t)}) \\
    \lambda_k ^{(t+1)}
        &= \lambda_k ^{(t)} + \rho \parens{z_k ^{(t+1)} - v_k ^{(t+1)}}, \quad k = 1, \ldots, p
\end{split}
\end{align}
In ADMM-based methods, these \(\mrm{update}\) procedures are ideally exact minimization, but sometimes this is not possible or practical.
In the following, we describe the updates for \(\gamma, v, z\) and the stopping condition.

\subsubsection{\(\gamma, v\)-Update}
We attempt to perform an approximate minimization by first ignoring the  \(\delta_{\mbb{R}_+} (\gamma)\) term and considering the following problem derived from~\eqref{eq:p3},
\begin{align*}
\begin{split}
    \underset{\gamma, v}{\text{minimize}}
        &\quad \frac{1}{2} \norm{\gamma}^2
            + \sum_{k = 1}^{p} \frac{\rho}{2} \xnorm{z_k ^{(t)} - v_k + \rho^{-1} \lambda_k ^{(t)}}^2 \\
    \text{subject to} &\quad z_\beta (\gamma) - \sum_{k = 1}^{p} H_k ^\top v_k = 0
\end{split}
\end{align*}
Using \(\rho x\) as the dual variable for this new problem, we derive the following optimality conditions
\begin{align}
    \label{eq:gamma-v-opt1}
    \begin{bmatrix} -D & J \\ J^\top & \rho^{-1} I \end{bmatrix}
    \begin{bmatrix} x \\ \gamma \end{bmatrix}
    &= \begin{bmatrix}
        - z_{\beta, 0} + \sum_{k = 1}^{p} H_k ^\top \parens{z_k ^{(t)} + \rho^{-1} \lambda_k ^{(t)}} \\
        0
    \end{bmatrix} \\
    \nonumber
    v_k &= z_k ^{(t)} + \rho^{-1} \lambda_k ^{(t)} + H_k x
\end{align}
where \(D = \sum_{k = 1}^{p} H_k ^\top H_k\).
The challenge, however is that the \(D\) and \(J\) matrices may not be full rank, and as such the matrix in the LHS of~\eqref{eq:gamma-v-opt1} may not be invertible.
Instead, we can derive a minimum-norm solution of \(x\) using the Moore-Penrose pseudoinverse in order to then express the \(v\) and \(\gamma\) updates as,
\begin{align*}
\begin{split}
    x &= - (D + \rho J J^\top)^{\dagger} \bigg(-z_{\beta, 0} + \sum_{k = 1}^{p} H_k ^\top \parens{z_k ^{(t)} + \rho^{-1} \lambda_k ^{(t)}} \bigg) \\
    v_k ^{(t+1)} &= z_k ^{(t)} + \rho^{-1} \lambda_k ^{(t)} + H_k x,
    \qquad
    \gamma^{(t+1)} = \Pi_{\mbb{R}_+} \bracks{- \rho J^\top x},
\end{split}
\end{align*}
where \(\Pi_{\mbb{R}_+}\) is projection onto the nonnegative orthant.


\subsubsection{\(z\)-Update}
Similar to before, we first ignore the \(\delta_{\mcal{S}_k} (z_k)\) terms and formulate the following unconstrained quadratic problem derived from~\eqref{eq:p3-lagrangian},
\begin{align*}
    \underset{z_1, \ldots, z_p}{\text{minimize}}
        &\quad \sum_{k = 1}^{p} \frac{\rho}{2} \xnorm{z_k - v_k ^{(t+1)} + \rho^{-1} \lambda^{(t)}}^2
\end{align*}
whose closed-form solutions we then project onto each \(\mbb{S}_{-} ^{\lvert \mcal{C}_k \rvert}\) and reshape into \(\mcal{S}_k\),
\begin{align*}
    z_k ^{(t+1)} = \mrm{vec}\parens{\Pi_{\mbb{S}_- ^{\lvert \mcal{C}_k \rvert}} \bracks{v_k ^{(t+1)} - \rho^{-1} \lambda_k ^{(t)}}}.
\end{align*}

\subsubsection{Stopping Condition}

\anton{Gotta play with the heuristics some more before we decide on a best one}


\subsection{Theoretical and Practical Concern}

{\color{blue}
\begin{itemize}
    \item We do not have or are aware of convergence guarantees for algorithms like this.
    
    \item However, any solution \(\gamma\) that the algorithm computes can be checked to see if indeed \(Z_\beta (\gamma) \preceq 0\).
    As such, our algorithm can be understood as a sound numerical heuristic.
    
    \item Caching aggressively helps.
    
    \item Block-index matrix operations can often be expanded into index manipulations.
\end{itemize}

}



==> contents/experiments-old.tex <==
\section{Numerical Experiments}
\label{sec:experiments}




We now evaluate the effectiveness of our approach, where we aim to answer the following:
(\textbf{Q1}) What is the scalability of our methods vs DeepSDP?
(\textbf{Q2}) How does \(\beta\) impact verification accuracy?
For accuracy experiments with DeepSDP see~\cite{fazlyab2020safety}, and recall that for a given \(\beta\), the formulations of DeepSDP, Chordal-DeepSDP, and Chordal-DeepSDP-2 are equivalent.


\paragraph*{QC Configuration}
For ReLU functions, we use the sector-bounded QC proposed in \cite[Lemma 4]{fazlyab2020safety} and for general sector-bounded activations we use that of \cite[Lemma 2]{fazlyab2020safety}.
Both of these have the same sparsity as \(Q_{\mrm{sec}}\) described in \eqref{eq:T-sector}.
We use \(Q_{\mrm{adj}}\) to encode interval propagation information that we obtain from the LiRPA library~\cite{xu2020automatic}, similar to the \emph{bounded nonlinearities} presented in~\cite[Section 3.C.4]{fazlyab2020safety}.
All of these activation QCs induce a \(Z(\gamma)\) with sparsity \(\mcal{E}_\beta\).


\paragraph*{Dataset}
As our primary focus is on improving the scalability of DeepSDP under parametrized sparsity, we use two randomly generated datasets in our experiments: one batch for \emph{scalability} experiments, and another batch for \emph{reachability} experiments.
We generate a collection of networks of widths \(= 10, 20\) and depths (\(K-1\)) \(= 5, 10, \ldots, 50\) with Gaussian random weights with \(\sigma \coloneqq 2 / \sqrt{w \log w}\) for scalability experiments and \(\sigma \coloneqq 1 / \sqrt{2}\) for reachability experiments.
We consider only ReLU activations.
For ease of plotting, each network has input and output dimensions \(n_1 \coloneqq m \coloneqq 2\).

\paragraph*{System}
All experiments were run on machines with Intel Xeon Gold 6148 CPU @ 2.40 GHz with 80 cores and 692 GB of RAM.
We used Julia 1.7.2~\cite{bezanson2017julia} for our implementation, and MOSEK 9.3~\cite{andersen2000mosek} as our convex solver.



\subsection{(\textbf{Q1}): Scalability}


For each random network we ran DeepSDP, Chordal-DeepSDP, and Chordal-DeepSDP-2 with \(\beta = 0, \ldots, 7\) to optimize a reachability ellipsoid when the initial input is constrained to the box \(\mcal{X} \coloneqq \{x : \norm{\mbf{1} - x}_\infty \leq 0.5\} \subseteq \mbb{R}^{2}\), where \(\mbf{1} \in \mbb{R}^2\) is the vector of ones.


\input{figures/scale-widths-plots}

Our plots are shown in Figure~\ref{fig:scale-widths-plots}.
We observe that Chordal-DeepSDP-2 consistently outperforms both DeepSDP and Chordal-DeepSDP, especially as the network depth increases.
While DeepSDP with \(\beta = 0\) is competitive, its performance quickly degrades as one increases \(\beta\) --- whereas the decay for Chordal-DeepSDP and Chordal-DeepSDP-2 is more gradual, meaning that we can achieve more accuracy without a significant performance penalty.





\input{figures/reach-plots}

\subsection{(\textbf{Q2}): Reachability}
We next investigate the impact of \(\beta\) on the verification accuracy.
We first fix an initial set to be the box \(\mcal{X} \coloneqq \{x : \norm{\mbf{1} - x}_\infty \leq 0.5\} \subseteq \mbb{R}^{2}\), where \(\mbf{1} \in \mbb{R}^2\) is the vector of ones.
Then, we uniformly sample \(10^{5}\) points to approximate the center \(y_c \in \mbb{R}^{2}\) and shape \(P \in \mbb{S}_+ ^{2}\) --- which is a regularized positive definite covariance matrix.
The reachability problem is to then minimize \(\rho\) subject to \(\norm{P^{-1} (y - y_c)}^2 \leq \rho\), for which \(S\) takes form described in \cite[Section 5.A]{fazlyab2020safety}.
Note that we fix \(P\) and \(y_c\) in contrast to the technique presented in~\cite{fazlyab2019probabilistic}, which allows for one to optimize over \(P\) and \(y_c\) directly at the cost of a larger semidefinite program.

We show the reach ellipsoids in Figure~\ref{fig:reach-plots} along with uniformly sampled outputs.
As the value of \(\beta\) increases, we see that the reach-set estimation becomes more accurate.





\subsection{Discussion}
Our experiments show that Chordal-DeepSDP-2 outperforms both DeepSDP and Chordal-DeepSDP on deep networks.
Moreover, both Chordal-DeepSDP and Chordal-DeepSDP-2 exhibit better scaling properties than DeepSDP as the value of \(\beta\) increases, with the performance of DeepSDP significantly degrading.

We found it helpful to run the dual formulation of DeepSDP, with help of the \texttt{Dualization.jl} library 
\footnote{
As of this writing, \texttt{Dualization.jl} does not yet support dualizing a feasibility primal problem.
We therefore add the simple objective of minimizing \(\norm{\gamma}^2\) for feasibility problems.
}
--- this alone achieves a very significant speedup (often over \(\times 10\)) compared to its primal formulation.
This same dualization trick does not seem to benefit Chordal-DeepSDP nor Chordal-DeepSDP-2, however, likely because of the large equality constraint that is not present in DeepSDP.



==> contents/future.tex <==
\section{Future Directions}
{\color{blue}

We list a few interesting directions below.

\subsection{Other Abstractions}
The accuracy of DeepSDP is dependent on what abstractions, especially of activation functions, are available.
Chiefly, a major innovation in the DeepSDP line of work~\cite{fazlyab2020safety,fazlyab2019efficient} are the development of \emph{sector-bounded} inequalities for neural network analysis.
New abstractions would help to improve the quality of verification.


\subsection{Polynomial Optimzation}
A promising recent development is the use of of polynomial optimization, specifically sum-of-squares~\cite{parrilo2000structured} techniques, for neural network verification~\cite{brown2022unified,chen2020semialgebraic,newton2021neural,newton2022sparse}.
Polynomial optimization allows for more expressive constraints than what is easily encodable in DeepSDP --- and thus the possibility of tighter verification results.
Common wisdom, however, is that sum-of-squares techniques often scale poorly because its fundamental computation is done using a very large SDP.
Exploiting problem-specific features~\cite{lofberg2009pre} and sparsity~\cite{newton2022sparse} are thus crucial for making polynomial optimization performant.
}


==> figures/reach-ellipbox.tex <==
\begin{figure}[h]
\centering
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=1.0\textwidth]{images/reach-ellipbox-x1-x2.png}
\end{subfigure}

\begin{subfigure}{0.45\textwidth}
\includegraphics[width=1.0\textwidth]{images/reach-ellipbox-x3-x4.png}
\end{subfigure}
\caption{
Bounds for \(\msf{Rand}\) with \(\beta = 0, \ldots, 10\).
}
\label{fig:reach-ellipbox}
\end{figure}


